A Non-linear Differentiable Model for Stormwater-based Irrigation of a Green Roof in Toronto

Green infrastructure has potential to alleviate the environmental impact of rapidly growing cities. This potential has inspired laws in Toronto that require the inclusion of rooftops with large vegetation beds, called green roofs, into sufficiently sized construction projects. We study the problem of reusing stormwater to irrigate a green roof in Toronto, where potable water is the current irrigation source. The vision is that widespread reuse of stormwater runoff for irrigation of green roofs and other purposes can reduce sewer overflow volumes without over-building (with the added benefit of conserving potable water). Towards this vision, our goal is to develop and evaluate two pump controllers for transporting stormwater to the green roof of interest in simulation. A key contribution is our development of a site-specific non-linear model for stormwater flow using smoothing techniques that permits linearization and a standard model predictive controller (MPC). We compare the efficacy of the MPC, which anticipates the weather, and an on/off controller, which is reactive rather than anticipative, for the site in simulation. With further study, we are hopeful that this research will advance control systems technology to improve the performance of green and stormwater infrastructure in growing urban areas.

==> old_linearization_notes.tex <==
The goal of linearization is to derive a dynamics equation of the form
\begin{subequations}\label{linearized}
\begin{equation}
    \tilde x_{t+1} = A_p \tilde x_t+ B_p \tilde u_t+ C_p\tilde w_{t,\text{r}} + D_p \tilde w_{t,\text{e}},
\end{equation}
where $p \coloneqq (\bar{x}_1, \bar{x}_2, \bar{u}, \bar{w}_\text{r}, \bar{w}_\text{e})$ is a current operating point, and the variables $\tilde x$, $\tilde u$, and $\tilde w$ are defined in terms of the operating point $p$ as follows:
\begin{equation}
    \tilde x  \coloneqq x - \bar{x}, \;\;\;  \tilde u  \coloneqq u - \bar{u}, \;\;\; \tilde w_\text{r} \coloneqq w_\text{r} - \bar{w}_\text{r}, \;\;\; \tilde w_\text{e} \coloneqq w_\text{e} - \bar{w}_\text{e}.
\end{equation}
Let $p \coloneqq (\bar{x_1}, \bar{x_2}, \bar{u}, \bar{w}_r, \bar{w}_e)$ be fixed. Also, let $u = \bar{u}$, $w_\text{r} = \bar{w_\text{r}}$, and $w_\text{e} = \bar{w_\text{e}}$. Let $(A_p, B_p, C_p)$ be the linearization of the model about the point $(\bar{x_1}, \bar{x_2}, \bar{u}, \bar{w_\text{r}}, \bar{w_\text{e}})$: 
\begin{equation}\label{linmodel}
\begin{gathered}
\left.
A_\text{p} =
\begin{bmatrix}
    \frac{\partial f_{01}}{\partial x_1} &  \frac{\partial f_{01}}{\partial x_2} \\
    \frac{\partial f_{02}}{\partial x_1} &  \frac{\partial f_{02}}{\partial x_2}
\end{bmatrix}
\right|_{p}
\text{, } 
\left.
B_\text{p} = 
\begin{bmatrix}
    \frac{\partial f_{01}}{\partial u}\\
    \frac{\partial f_{02}}{\partial u}
\end{bmatrix}
\right|_{p}
\text{, }
\left.
C_\text{p} = 
\begin{bmatrix}
    \frac{\partial f_{01}}{\partial w_r}\\
    \frac{\partial f_{02}}{\partial w_r}
\end{bmatrix}
\right|_{p} \\
\left.
D_\text{p} = 
\begin{bmatrix}
    \frac{\partial f_{01}}{\partial w_e}\\
    \frac{\partial f_{02}}{\partial w_e}
\end{bmatrix}
\right|_{p}
\end{gathered}
\end{equation}
\end{subequations}
Let $a$ be a fixed number (e.g., $a = 100$ m\textsuperscript{3}). We want to plot:
\begin{enumerate}
    \item $g_{\text{L}}(x) \coloneqq \bar{x} + A_p \tilde x+ B_p \tilde u+ C_p\tilde w_r + D_p \tilde w_e$ versus \\$x \in [\bar{x}-a, \bar{x}+a]$,
    \item $g_{\text{N}}(x) \coloneqq x + f^\epsilon(x, u, w) \Delta \tau$ versus \\$x \in [\bar{x}-a, \bar{x}+a]$.
\end{enumerate}
We repeat the above procedure for different choices of $\bar{x}$. The linearization of $f$ around different operating points $p$ are shown in Fig. \ref{linearization}.
\begin{figure}[ht]
% \the\columnwidth
\centerline{\includegraphics[width=\columnwidth]{model_figures/linearized/all_linearizedfig.png}}
\caption{Linearization of $f^{\epsilon}_{1}$ around different choices of $p$. \textcolor{blue}{It is nice to show these plots. It might better to show the vertical axis slightly more zoomed out. It is a bit hard to see the title/y-axis labels/etc. It may be better to write $p = (125, 0, 20, 9.5 \cdot 10^{-xx})$ without so many zeros to provide more room. Or, the title instead can include ``$...p = p_1$'' and then we define $p_1$ in the caption. We would like the size the numbers/labels etc. to be no smaller than the size of the font in the caption. We don't need to write $f_{01}$ anymore -- writing $f_1$ is fine.}}
\label{linearization}
\end{figure}

==> revisions/my_file_v1.tex <==
The system consists of an underground cistern and a rooftop vegetation. Two pumps connected in parallel pump water from the cistern to the rooftop for irrigation purposes.

Let $t \in \mathbb{T} := \{0,1,...,N-1\}$ be given. If $x_t \in S$, $u_t \in A$, and $w_t \in \mathbb{R}$ are the values of $X_t$, $U_t$, and $W_t$, respectively, then the value of $X_{t+1}$ is given by
\begin{subequations}\label{dynwater}
\begin{equation}\begin{aligned}
    x_{t+1} = x_t + f_0(x_t,u_t,w_t)\cdot \triangle\tau,
\end{aligned}\end{equation}
such that if $x_{t+1,i} \geq \overline{k}_i$, then we redefine $x_{t+1,i} \coloneqq \overline{k}_i$, where $x_\text{t,i} \in [0, \overline{k}_{i}]$ (m\textsuperscript{3}) is the water volume of tank $i$. $u_{t} \in [0, v_\text{max}]$ is a pump setting, which is a value of $U_t$. $w_{t} \in \mathbb{R}$ is a value of the random disturbance $W_{t}$, representing surface runoff that enters the system during the storm. 

The function $f_0 : \mathbb{R}_+^2 \times A \times \mathbb{R} \rightarrow \mathbb{R}_+^2$ is chosen according to simplified Newtonian physics:
\begin{equation}\label{physics}\begin{aligned}
f_0(x,u,w) & \coloneqq \left[ f_{01}(x,u,w), f_{02}(x,u,w) \right]^{T},\\
f_{01}(x,u,w) & \coloneqq  w - q_{\text{out}}(x_{1}) - q_\text{pump}(x,u),\\
f_{02}(x,u,w) & \coloneqq  w + q_\text{pump}(x,u)  - q_\text{evap} \\
\end{aligned}\end{equation}

We will define $q_\text{out}$, $q_\text{pump}$, $q_\text{evap}$, subsequently. Please refer to Table I for a list of model parameters.

The cistern is equipped with an outlet that allows water to drain down via gravity when its water level reaches $z_\text{o}$. The flow rate of the water leaving the cistern via the outlet is defined by $q_\text{out}$, with an outlet radius $r_\text{o}$ and elevation $z_\text{o}$.
\begin{equation}\label{physics-out}\begin{aligned}
%q_\text{out}(x_{1}) & \coloneqq \bar{q_{o}}(x_{1}) - \frac{\bar{q_{o}}(x_{1})}{\bar{x_{1}}-z_{o}} \cdot \min(\bar{x_{1}}-\frac{x_{1}}{A_{1}}, \bar{x_{1}}-z_{o}),\\
%\overline{q}_\text{o}(x_{1}) &:= c_\text{d} \bar{\pi} r_\text{o}^2 \sqrt{2 \tilde{g} \frac{x_{1}}{A_{1}}},\\
q_\text{out}(x_{1}) &:= \begin{cases} c_\text{d} \tilde{\pi} r_\text{o}^2 \sqrt{2 \tilde{g} \frac{x_{1}}{A_{1}}}, & \text{if } \frac{x_{1}}{A_{1}} \geq z_o \\0 & \text{otherwise} \end{cases},\\
\end{aligned}\end{equation}

The flow rate of the pump, $q_\text{pump}(x,u)$, is derived from linear approximations of pump performance curves as well as the total head loss of the system. The system has pumps arranged in series to pump water from the cistern to the rooftop vegetation, therefore the slope of the linear approximated pump performance curves were doubled. The total head loss of the system is defined as the sum of the total static head loss, friction head loss, and the minor losses in the pipe system. The total static head loss is the total vertical distance that the water is raised by the pump. The friction head loss and minor head loss were determined based on the geometry and size of the pipe system, using the equation given in \cite[Eq. 6.79, p. 389]{white2011fluid}. 
The expression for $q_\text{pump}(x,u)$ is given by (\ref{physics-pump}), where $u$ is the control input of the speed of pump, $v_\text{max}$ is the maximum operating speed of pump, $z_\text{H}$ is the required net positive suction head of the pump, and $z_\text{veg}$ is the minimum water balance required in the rooftop vegetation soil. 
%and $C_\text{pump}$ is the unit conversion factor that converts the flow rate from $\frac{\text{gallons}}{\text{min}}$ to $\frac{\text{m}\textsuperscript{3}}{\text{s}}$. 

\begin{equation}\label{physics-pump}\begin{aligned}
q_{\text{pump}}(x,u) &:= \begin{cases} 0 & \text{if }
\frac{x_{2}}{A_{2}} \geq z_\text{veg} \text{ or} \\ 
\text{} & \frac{x_{1}}{A_{1}} - z_\text{pump} < z_\text{H}\\
\frac{u}{v_{\text{max}}} \cdot \bar{q}_{\text{pump},v_{\text{max}}}(x) & \text{otherwise} \end{cases} \\
\end{aligned}\end{equation}

\begin{equation}\label{physics-pump-sub}\begin{aligned}
\bar{q}_{\text{pump},v_{\text{max}}}(x) & \coloneqq \frac{-\Delta_\text{pump}+ \sqrt{\Delta_\text{pump}^2-4c_{1}(\frac{x_{2}^2}{A_{2}}+d- \frac{x_{1}^2}{A_{1}}-H_\text{pump,0})}}{2c_{1}}\\
c_{1} & \coloneqq \frac{f \frac{l}{D} + k_\text{L}}{2 \tilde{g} a_{\text{pump}}} \\
z_\text{H} & \coloneqq c_\text{H,1} \cdot (c_\text{H,2})^{q_\text{pump}}\\
\end{aligned}\end{equation}

%The evaporation rate of the plants on tank 2 is modelled using $q_\text{evap}$, where $e$ is the evaporation coefficient ($\frac{\text{kg}} {\text{m\textsuperscript{2}hr}}$), $h$ is the xxx and $h_\text{max}$ [2].
The evaporation rate of the rooftop vegetation is modelled with $q_\text{evap}$, which is derived from the FAO-56 Penman-Monteith Equation, where $E$ is the evapotranspiration rate of vegetation ($\frac{\text{mm}}{\text{day}}$) \cite[Eq. 4, p. 2]{zotarelli2010step}. A unit conversion factor $c_\text{evap}$ is multiplied to convert the units of $E$ from $\frac{\text{mm}}{\text{day}}$ to $\frac{\text{m}}{\text{s}}$. 
%$\Delta$ represents the slope of saturation vapour pressure at the mean temperature, $T_\text{mean}$ \cite[Eq. 9, p. 4]{zotarelli2010step}.
\begin{equation}\label{physics-evap}\begin{aligned}
%.  q_{\text{evap}} & \coloneqq \frac{eA_{2}(h_{\text{max}}-h)}{3600000},\\
%.  e & \coloneqq 25+19v_{\text{air}}
%.  q_\text{storm,2}(x) &:= \begin{cases} c_\text{d} \bar{\pi} r_\text{d}^2 \sqrt{2 \tilde{g} (x_2 - z_2)} & \text{if } x_2 \geq z_2 \\0 & \text{otherwise} \end{cases}.
q_\text{evap} & \coloneqq A_{2} \cdot c_\text{evap} \cdot E \\
%E & \coloneqq \frac{0.408 \Delta (R_\text{n}-G)+ \gamma \frac{900}{T_\text{mean}+273}v_\text{wind}(e_\text{s}-e_\text{a})}{\Delta + \gamma (1+0.34v_\text{wind})} \\
\end{aligned}\end{equation}

%\begin{equation}\label{physics-evap-delta}\begin{aligned}
%\Delta & \coloneqq \frac{4098[0.6108 %\exp{\frac{17.27T_\text{mean}}{T_\text{mean}+237.3}}]}{(T_\text{mean}+237.3)^2}
%\end{aligned}\end{equation}

%The psychrometric constant, $\gamma$ ($\frac{\text{kPa}}{\celsius}$), is described with equation (\ref{physics-evap-gamma}).\\
%\begin{equation}\label{physics-evap-gamma}\begin{aligned}
%\gamma & \coloneqq \frac{C_\text{p}P}{\epsilon \lambda}\\
%\end{aligned}\end{equation}

%$e_\text{s}$ (kPa) is the mean vapour pressure obtained from the saturation vapour pressure at daily minimum and maximum temperatures in \celsius. They are represented as $e_{(T_\text{min})}$ and $e_{(T_\text{max})}$ respectively. $T_\text{min}$ and $T_\text{max}$ are obtained from \cite{canada_2021}.

%$e_\text{a}$ (kPa) is the actual vapour pressure. It is set to be equivalent to $e_{(T_\text{min})}$ when the dew point temperature is relatively close to $T_\text{min}$ \cite[p. 6]{zotarelli2010step}. 

%\begin{equation}\label{physics-evap-e}\begin{aligned}
%e_\text{s} & \coloneqq \frac{e_{(T_\text{min})}+e_{(T_\text{max})}}{2}\\
%e_{(T_\text{min})} & \coloneqq 0.6108 \exp{(\frac{17.27T_\text{min}}{T_\text{min}+237.3})}\\
%e_{(T_\text{max})} & \coloneqq 0.6108 \exp{(\frac{17.27T_\text{max}}{T_\text{max}+237.3})}\\
%e_\text{a} & \coloneqq e_{(T_\text{min})}
%\end{aligned}\end{equation}
\end{subequations}
%
Table \ref{tanksysinfo} lists model parameters.

\begin{table}[ht]
\caption{Stormwater System Parameters (Baseline)}
\label{table}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{|p{25pt}|p{125pt}|p{63pt}|}
\hline
\textbf{Symbol} &  \textbf{Description} & \textbf{Value} \vspace{.5mm}\\
\hline
%$a_1$ & Surface area of cistern & xxx [m\textsuperscript{2}] \vspace{.6mm}\\
%$a_2$ & Surface area of rooftop vegetation & xxx [m\textsuperscript{2}] %\vspace{.6mm}\\
$A_1$ & Bottom surface area of cistern & 7.2 [m\textsuperscript{2}] \vspace{.6mm}\\
$A_2$ & Bottom surface area of rooftop vegetation& 68.8 [m\textsuperscript{2}] \vspace{.6mm}\\
$a_\text{pump}$ & Area of flow through pump & 0.01 $\tilde{\pi}$ [m\textsuperscript{2}] \vspace{.6mm}\\
%
$c_\text{d}$ & Discharge coefficient & 0.61 (no units) \vspace{.6mm}\\
$c_\text{evap}$ & Unit conversion factor for rooftop evapotranspiration rate & $1.16\mathrm{e}{-8}$ [$\frac{\frac{m}{mm}}{\frac{s}{day}}$] \vspace{.6mm} \\
% 0.0116 
$c_\text{H,1}$ & Constant of the pump's required NPSH curve & 2.288 (no units)\vspace{.6mm}\\
$c_\text{H,2}$ & Constant of the pump's required NPSH curve & 1.17 (no units)\vspace{.6mm}\\
%$C_\text{p}$ & Specific heat at constant pressure & $1.013\mathrm{e}{-3}$ [$\frac{\text{MJ}}{\text{kg}\text{\celsius}}$] \vspace{.6mm} \\
%$c_\text{pump}$ & Unit conversion factor for pump flow rate & $6.31\mathrm{e}{-5}$ [$\frac{\frac{m^3}{gal}}{\frac{s}{min}}$] \vspace{.6mm} \\
%
$d$ & Elevation of rooftop vegetation relative to the cistern & 16 [m] \vspace{.6mm}\\
$D$ & Diameter of pipe & 0.2 [m] \vspace{.6mm}\\
$\Delta_\text{pump}$ & Magnitude of slope of pump performance equation & 5400 [$\frac{m}{\frac{m^3}{s}}$] \vspace{.6mm}\\
%
%$e_\text{s}$ & Mean saturation vapour pressure derived from air temperature & kPa \vspace{.6mm}\\
%$e_\text{a}$ & Actual vapour pressure derived from relative humidity & kPa \vspace{.6mm}\\
%$\epsilon$ & Ratio molecular weight of water vapour & 0.622 \vspace{.6mm}\\
%
$f$ & Friction factor of pipe system & $\approx$3.55 \vspace{.6mm}\\
%
$\tilde{g}$ & Acceleration due to gravity & 9.81 $\frac{\text{m}}{\text{s}^2}$ \vspace{.6mm}\\
%$G$ & Soil heat flux density & 0.4 $\frac{\text{MJ}}{\text{m}^2\text{day}}$\vspace{.6mm}\\
%
%$h$ & Humidity ratio of air & \text{From Toronto weather} \vspace{.6mm} \text{data \cite{canada_2021}} \vspace{.6mm}\\
%$h_\text{max}$ & Maximum humidity ratio of saturated air & 0.019826 at 25 \degree $C$ \vspace{.6mm}\\
$H_\text{pump,0}$ & Pump head in series at 0 flow rate & 59.7 m \vspace{.6mm}\\
%${k}_1$ & Water level in tank 1 & \vspace{.6mm}\\
%
%$\overline{k}_1$ & Maximum value of water level in tank 1 & 4 m \vspace{.6mm}\\
%
$k_\text{L}$ & Minor loss coefficient of system & 0.6 \vspace{.6mm}\\
%
$l$ & Length of pipe & 18.4 m \vspace{.6mm}\\
%$\lambda$ & Latent heat of vaporization & 2.45 
%$\frac{\text{MJ}}{\text{kg}}$ \vspace{.6mm}\\
%
$N$ & Length of discrete time horizon & 20 ($=$ 1 h) \vspace{.6mm}\\
%
%$P$ & Atmospheric pressure at 12 m above sea level & 101.16 kPa \vspace{.6mm}\\
$\tilde{\pi}$ & Circle circumference-to-diameter ratio & $\approx$3.14 \vspace{.6mm}\\
%
$r_\text{o}$ & Radius of outlet in cistern & $0.125$ m \vspace{.6mm}\\
%$R_\text{n}$ & Net radiation flux & \text{From Natural Resources} \vspace{.6mm} \text{Canada $\frac{\text{MJ}}{\text{m}^2\text{(day)}}$  \cite{canada_2020}} \vspace{.6mm}\\
%

$ \triangle \tau $ & Duration of $[t,t+1)$ & 3 min \vspace{.6mm}\\
%
%$v_\text{max}$ & Maximum operating speed of pump & 3450 rpm \vspace{.6mm}\\
%$v_\text{wind}$ & Wind speed & Stochastically generated $\frac{\text{m}}{\text{s}}$ \vspace{.6mm}\\
%$v_\text{air}$ & Velocity of air above water surface & 0.5 m/s \vspace{.6mm}\\
%
$z_\text{H}$ & Net positive suction head required in cistern & m \\
$z_\text{o}$ & Elevation of outlet in cistern & 1.29 m \vspace{.6mm}\\
$z_\text{pump}$ & Pump elevation w.r.t base of cistern & 0.15 m \vspace{.6mm}\\
$z_\text{veg}$ & Minimum water balance required for rooftop vegetation & $4.57\mathrm{e}{-2}$ \cite{melvin_yonts_2009} \vspace{.6mm} \\
%
\hline
\multicolumn{3}{p{251pt}}{m $=$ meter, s $=$ 
seconds, min $=$ minutes, h $=$ hours, rpm $=$ revolutions per minute, MJ $=$ mega-joules, kPa $=$ kilo-pascals.}
\end{tabular}
\label{tanksysinfo}
\end{table}

\begin{figure}[th]
% \the\columnwidth
\centerline{\includegraphics[width=\columnwidth]{cistern_rooftop3.png}}
\caption{This is the figure caption}
\label{exptfigure}
\end{figure}

\subsection{Smooth approximation of system equations}
Smooth approximation algorithms mentioned in \cite{duan_lian_2016} are applied to equation (\ref{physics}).
With all definitions following from section \ref{main-model}, we redefine the value of $X_{t+1}$ to be
\begin{equation}\label{linear}
x_{t+1} = x_t + f_{0}^{\epsilon}(x_t, u_t, w_t) \cdot \triangle\tau 
\end{equation}

Where $f_0^{\epsilon}(x_t,u_t,w_t)$ is smooth approximated $f_0(x_t,u_t,w_t)$.
\begin{equation}\label{physics}\begin{aligned}
f_0^{\epsilon}(x,u,w) & \coloneqq \left[ f_{01}^{\epsilon}(x,u,w), f_{02}^{\epsilon}(x,u,w) \right]^{T},\\
f_{01}^{\epsilon}(x,u,w) & \coloneqq  w - q_{\text{out}}^{\epsilon}(x_{1}) - q_\text{pump}^{\epsilon}(x,u),\\
f_{02}(x,u,w) & \coloneqq  w + q_\text{pump}^{\epsilon}(x,u)  - q_\text{evap} \\
\end{aligned}\end{equation}

First, from equation (\ref{physics-out}), we define a smooth approximation of $q_\text{out}(x_1)$ to be $q_\text{out}^{\epsilon}(x_1)$, where $\epsilon$ is a small positive real number.
\begin{subequations}\label{smooth}
\begin{equation}\label{smooth-physics-out}
%c_\text{out} & \coloneqq c_\text{d} \tilde{\pi} r_\text{o}^2 \sqrt{2 \tilde{g}}\\
q_\text{out}^{\epsilon}(x_1) := \begin{cases} c_\text{out} \frac{2}{3} \sqrt{\epsilon} & \text{if } \frac{x_{1}}{A_{1}}<z_\text{o} \\ c_\text{out} (\frac{1}{3} \epsilon^{-1} (x_1)^{\frac{3}{2}} + \frac{2}{3} \sqrt{\epsilon}) & \\ \hspace{10mm} \text{if } z_\text{o} < \frac{x_1}{A_1} \leq z_\text{o}+\epsilon \\ c_\text{out} \sqrt{x_1} & \text{if } \frac{x_1}{A_1} > z_\text{o} + \epsilon \end{cases}
\end{equation}
\begin{equation}\label{cout}
c_\text{out} \coloneqq c_\text{d} \tilde{\pi} r_\text{o}^2 \sqrt{\frac{2\tilde{g}}{A_1}}
\end{equation}

Then, from equation (\ref{physics-pump}), we define a smooth approximation of (\ref{physics-pump-sub}) to be $\bar{q}_{\text{pump},v_{\text{max}}}^{\epsilon}(x)$.
\begin{equation}\label{smooth-physics-pump-sub}
\bar{q}_{\text{pump},v_{\text{max}}}^{\epsilon}(x) \coloneqq \frac{-\Delta_\text{pump} + \bar{q}^{\epsilon}(x)}{2c_1}
\end{equation}
\begin{equation}\label{q-epsilon}
\bar{q}^{\epsilon}(x) \coloneqq \begin{cases} \frac{2}{3} \sqrt{\epsilon} & \\ \text{\hspace{8mm} if } c_\text{pump} - 4 c_1 (\frac{x_2^2}{A_2} - \frac{x_1^2}{A_1}) \leq 0 \\ \text{} \\ \frac{1}{3} \epsilon^{-1} (c_\text{pump} - 4 c_1 (\frac{x_2^2}{A_2} - \frac{x_1^2}{A_1})) + \frac{2}{3} \sqrt{\epsilon} & \\  \text{\hspace{8mm} if } 0 < c_\text{pump} - 4 c_1 (\frac{x_2^2}{A_2} - \frac{x_1^2}{A_1}) \leq \epsilon \\ \text{} \\ \sqrt{c_\text{pump} - 4 c_1 (\frac{x_2^2}{A_2} - \frac{x_1^2}{A_1})} & \\ \text{\hspace{8mm} if } c_\text{pump} - 4 c_1 (\frac{x_2^2}{A_2} - \frac{x_1^2}{A_1}) > \epsilon \end{cases}
\end{equation}
\begin{equation}
    c_\text{pump} \coloneqq \Delta_\text{pump}^2 - 4c_1 d + 4 c_1 H_\text{pump,0}
\end{equation}
\end{subequations}

\subsection{Linearization of smoothed system equations}


\section{Model predictive control idea}
Suppose that $t$ is the current time, $x$ is the state at time $t$, $u$ is the control at time $t-1$, and $w$ is the average disturbance during the time horizon $\{t-M,t-M+1,...,t\}$, that is, $w = \frac{1}{M+1}\sum_{j = t-M}^t w_j$.
\begin{enumerate}
    \item Linearize the model around $(x,u,w)$ to obtain matrices $(A_t,B_t,C_t, a_t)$. $A_t \in \mathbb{R}^{2 \times 2}$, $B_t \in \mathbb{R}^{2 \times 1}$, $C_t \in \mathbb{R}^{2 \times 1}$, and $a_t \in \mathbb{R}^{2 \times 1}$ such that
    \begin{equation}
        x_{t+1} = A_t x_t + B_t u_t + C_t w_t + a_t
    \end{equation}
    for all $(x_t,u_t,w_t)$ ``close to'' $(x,u,w)$.
    \item Find $(w_t,w_{t+1},w_{t+2},...,w_{t+N})$ from the forecast.
    \item Find $(u_j)_{j = t}^{t+N} := (u_t,u_{t+1},u_{t+2},...,u_{t+N})$ to minimize the cost 
    \begin{subequations}
    \begin{equation}\label{cost}
        J((u_j)_{j = t}^{t+N}) := \sum_{i=t}^{t+N} (x_{i2}/A_2 - t_\text{veg})^2 + \lambda u_i^2,
    \end{equation}
    subject to 
    \begin{equation}
        x_{i+1} = A_i x_i + B_i u_i + C_i w_i + a_i, \;\;\; i = t, t+1,...,t+N.
    \end{equation}
    \end{subequations}
    The parameter $\lambda \geq 0$ is chosen to trade-off the desire to keep $x_{i2}/A_2$ close to $t_\text{veg}$ (so that the plants have enough water) and to conserve energy that is used by the pump ($|u_i|$ higher means that the pump requires more energy to operate).
    \item Apply $u_t$.
    \item Proceed to the next time step, i.e., update $t$ by 1.
    \item Proceed to step 1 if we are still within desired time horizon. 
\end{enumerate}
Compare the cost \eqref{cost} that we get from the algorithm above to a simple/baseline controller (if it will rain today with 80\% probability, then do not pump. Otherwise, pump water at a constant rate.)

%%\bar{q}^{\epsilon}(x) \coloneqq \begin{cases} \frac{2}{3} \sqrt{\epsilon} & \\ \text{\hspace{8mm} if } c_\text{pump} - 4 c_1 (\frac{x_2^2}{A_2} - \frac{x_1^2}{A_1}) \leq 0 \\ \text{} \\ \frac{1}{3} \epsilon^{-1} (c_\text{pump} - 4 c_1 (\frac{x_2^2}{A_2} - \frac{x_1^2}{A_1})) + \frac{2}{3} \sqrt{\epsilon} & \\  \text{\hspace{8mm} if } 0 < c_\text{pump} - 4 c_1 (\frac{x_2^2}{A_2} - \frac{x_1^2}{A_1}) \leq \epsilon \\ \text{} \\ \sqrt{c_\text{pump} - 4 c_1 (\frac{x_2^2}{A_2} - \frac{x_1^2}{A_1})} & \\ \text{\hspace{8mm} if } c_\text{pump} - 4 c_1 (\frac{x_2^2}{A_2} - \frac{x_1^2}{A_1}) > \epsilon \end{cases}

==> revisions/my_file_v2_with_qevap_and_linear.tex <==
The system consists of an underground cistern and a rooftop vegetation. Two pumps connected in parallel pump water from the cistern to the rooftop for irrigation purposes.

Let $t \in \mathbb{T} := \{0,1,...,N-1\}$ be given. If $x_t \in S$, $u_t \in A$, and $w_t \in \mathbb{R}$ are the values of $X_t$, $U_t$, and $W_t$, respectively, then the value of $X_{t+1}$ is given by
\begin{subequations}\label{dynwater}
\begin{equation}\begin{aligned}
    x_{t+1} = x_t + f_0(x_t,u_t,w_t)\cdot \triangle\tau,
\end{aligned}\end{equation}
such that if $x_{t+1,i} \geq \overline{k}_i$, then we redefine $x_{t+1,i} \coloneqq \overline{k}_i$, where $x_\text{t,i} \in [0, \overline{k}_{i}]$ (m\textsuperscript{3}) is the water volume of tank $i$. $u_{t} \in [0, v_\text{max}]$ is a pump setting, which is a value of $U_t$. $w_{t} \in \mathbb{R}$ is a value of the random disturbance $W_{t}$, representing surface runoff that enters the system during the storm. 

The function $f_0 : \mathbb{R}_+^2 \times A \times \mathbb{R} \rightarrow \mathbb{R}_+^2$ is chosen according to simplified Newtonian physics:
\begin{equation}\label{physics-smooth}\begin{aligned}
f_0(x,u,w) & \coloneqq \left[ f_{01}(x,u,w), f_{02}(x,u,w) \right]^{T},\\
f_{01}(x,u,w) & \coloneqq  w - q_{\text{out}}(x_{1}) - q_\text{pump}(x,u),\\
f_{02}(x,u,w) & \coloneqq  w + q_\text{pump}(x,u)  - q_\text{evap} \\
\end{aligned}\end{equation}

We will define $q_\text{out}$, $q_\text{pump}$, $q_\text{evap}$, subsequently. Please refer to Table I for a list of model parameters.

The cistern is equipped with an outlet that allows water to drain down via gravity when its water level reaches $z_\text{o}$. The flow rate of the water leaving the cistern via the outlet is defined by $q_\text{out}$, with an outlet radius $r_\text{o}$ and elevation $z_\text{o}$.
\begin{equation}\label{physics-out}\begin{aligned}
%q_\text{out}(x_{1}) & \coloneqq \bar{q_{o}}(x_{1}) - \frac{\bar{q_{o}}(x_{1})}{\bar{x_{1}}-z_{o}} \cdot \min(\bar{x_{1}}-\frac{x_{1}}{a_{1}}, \bar{x_{1}}-z_{o}),\\
%\overline{q}_\text{o}(x_{1}) &:= c_\text{d} \bar{\pi} r_\text{o}^2 \sqrt{2 \tilde{g} \frac{x_{1}}{a_{1}}},\\
q_\text{out}(x_{1}) &:= \begin{cases} c_\text{d} \tilde{\pi} r_\text{o}^2 \sqrt{2 \tilde{g} \frac{x_{1}}{a_{1}}}, & \text{if } \frac{x_{1}}{a_{1}} \geq z_o \\0 & \text{otherwise} \end{cases},\\
\end{aligned}\end{equation}

The flow rate of the pump, $q_\text{pump}(x,u)$, is derived from linear approximations of pump performance curves as well as the total head loss of the system. The system has pumps arranged in series to pump water from the cistern to the rooftop vegetation, therefore the slope of the linear approximated pump performance curves were doubled. The total head loss of the system is defined as the sum of the total static head loss, friction head loss, and the minor losses in the pipe system. The total static head loss is the total vertical distance that the water is raised by the pump. The friction head loss and minor head loss were determined based on the geometry and size of the pipe system, using the equation given in \cite[Eq. 6.79, p. 389]{white2011fluid}. 
The expression for $q_\text{pump}(x,u)$ is given by (\ref{physics-pump}), where $u$ is the control input of the speed of pump, $v_\text{max}$ is the maximum operating speed of pump, $z_\text{H}$ is the required net positive suction head of the pump, and $z_\text{veg}$ is the minimum water balance required in the rooftop vegetation soil. 
%and $C_\text{pump}$ is the unit conversion factor that converts the flow rate from $\frac{\text{gallons}}{\text{min}}$ to $\frac{\text{m}\textsuperscript{3}}{\text{s}}$. 

\begin{equation}\label{physics-pump}\begin{aligned}
q_{\text{pump}}(x,u) &:= \begin{cases} 0 & \text{if }
\frac{x_{2}}{a_{2}} \geq z_\text{veg} \text{ or} \\ 
\text{} & \frac{x_{1}}{a_{1}} - z_\text{pump} < z_\text{H}\\
\frac{u}{v_{\text{max}}} \cdot \bar{q}_{\text{pump},v_{\text{max}}}(x) & \text{otherwise} \end{cases} \\
\end{aligned}\end{equation}

\begin{equation}\label{physics-pump-sub}\begin{aligned}
\bar{q}_{\text{pump},v_{\text{max}}}(x) & \coloneqq \frac{-\Delta_\text{pump}+ \sqrt{\Delta_\text{pump}^2-4c_{1}(d- \frac{x_{1}}{a_{1}}-H_\text{pump,0})}}{2c_{1}}\\
c_{1} & \coloneqq \frac{f \frac{l}{D} + k_\text{L}}{2 \tilde{g} a_{\text{pump}}} \\
%z_\text{H} & \coloneqq c_\text{H,1} \cdot (c_\text{H,2})^{q_\text{pump}}\\
\end{aligned}\end{equation}

%The evaporation rate of the plants on tank 2 is modelled using $q_\text{evap}$, where $e$ is the evaporation coefficient ($\frac{\text{kg}} {\text{m\textsuperscript{2}hr}}$), $h$ is the xxx and $h_\text{max}$ [2].
The evaporation rate of the rooftop vegetation is modelled with $q_\text{evap}$, which is derived from the FAO-56 Penman-Monteith Equation, where $E$ is the evapotranspiration rate of vegetation ($\frac{\text{mm}}{\text{day}}$) \cite[Eq. 4, p. 2]{zotarelli2010step}. 
%A unit conversion factor $c_\text{evap}$ is multiplied to convert the units of $E$ from $\frac{\text{mm}}{\text{day}}$ to $\frac{\text{m}}{\text{s}}$. 

%$\Delta$ represents the slope of saturation vapour pressure at the mean temperature, $T_\text{mean}$ \cite[Eq. 9, p. 4]{zotarelli2010step}.
%\begin{equation}\label{physics-evap}\begin{aligned}
%.  q_{\text{evap}} & \coloneqq \frac{ea_{2}(h_{\text{max}}-h)}{3600000},\\
%.  e & \coloneqq 25+19v_{\text{air}}
%.  q_\text{storm,2}(x) &:= \begin{cases} c_\text{d} \bar{\pi} r_\text{d}^2 \sqrt{2 \tilde{g} (x_2 - z_2)} & \text{if } x_2 \geq z_2 \\0 & \text{otherwise} \end{cases}.
%q_\text{evap} & \coloneqq a_{2} \cdot c_\text{evap} \cdot E \\
%E & \coloneqq \frac{0.408 \Delta (R_\text{n}-G)+ \gamma \frac{900}{T_\text{mean}+273}v_\text{wind}(e_\text{s}-e_\text{a})}{\Delta + \gamma (1+0.34v_\text{wind})} \\
%\end{aligned}\end{equation}

%\begin{equation}\label{physics-evap-delta}\begin{aligned}
%\Delta & \coloneqq \frac{4098[0.6108 %\exp{\frac{17.27T_\text{mean}}{T_\text{mean}+237.3}}]}{(T_\text{mean}+237.3)^2}
%\end{aligned}\end{equation}

%The psychrometric constant, $\gamma$ ($\frac{\text{kPa}}{\celsius}$), is described with equation (\ref{physics-evap-gamma}).\\
%\begin{equation}\label{physics-evap-gamma}\begin{aligned}
%\gamma & \coloneqq \frac{C_\text{p}P}{\epsilon \lambda}\\
%\end{aligned}\end{equation}

%$e_\text{s}$ (kPa) is the mean vapour pressure obtained from the saturation vapour pressure at daily minimum and maximum temperatures in \celsius. They are represented as $e_{(T_\text{min})}$ and $e_{(T_\text{max})}$ respectively. $T_\text{min}$ and $T_\text{max}$ are obtained from \cite{canada_2021}.

%$e_\text{a}$ (kPa) is the actual vapour pressure. It is set to be equivalent to $e_{(T_\text{min})}$ when the dew point temperature is relatively close to $T_\text{min}$ \cite[p. 6]{zotarelli2010step}. 

%\begin{equation}\label{physics-evap-e}\begin{aligned}
%e_\text{s} & \coloneqq \frac{e_{(T_\text{min})}+e_{(T_\text{max})}}{2}\\
%e_{(T_\text{min})} & \coloneqq 0.6108 \exp{(\frac{17.27T_\text{min}}{T_\text{min}+237.3})}\\
%e_{(T_\text{max})} & \coloneqq 0.6108 \exp{(\frac{17.27T_\text{max}}{T_\text{max}+237.3})}\\
%e_\text{a} & \coloneqq e_{(T_\text{min})}
%\end{aligned}\end{equation}
\end{subequations}
%
Table \ref{tanksysinfo} lists model parameters.

\begin{table}[ht]
\caption{Stormwater System Parameters (Baseline)}
\label{table}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{|p{25pt}|p{125pt}|p{63pt}|}
\hline
\textbf{Symbol} &  \textbf{Description} & \textbf{Value} \vspace{.5mm}\\
\hline
%$a_1$ & Surface area of cistern & xxx [m\textsuperscript{2}] \vspace{.6mm}\\
%$a_2$ & Surface area of rooftop vegetation & xxx [m\textsuperscript{2}] %\vspace{.6mm}\\
$a_1$ & Bottom surface area of cistern & 70 [m\textsuperscript{2}] \vspace{.6mm}\\
$a_2$ & Bottom surface area of rooftop vegetation& 68.8 [m\textsuperscript{2}] \vspace{.6mm}\\
$a_\text{pump}$ & Area of flow through pump & 0.01 $\tilde{\pi}$ [m\textsuperscript{2}] \vspace{.6mm}\\
%
$c_\text{d}$ & Discharge coefficient & 0.61 (no units) \vspace{.6mm}\\
% $c_\text{evap}$ & Unit conversion factor for rooftop evapotranspiration rate & $1.16\mathrm{e}{-8}$ [$\frac{\frac{m}{mm}}{\frac{s}{day}}$] \vspace{.6mm} \\
% 0.0116 
$c_\text{H,1}$ & Constant of the pump's required NPSH curve & 2.288 (no units)\vspace{.6mm}\\
$c_\text{H,2}$ & Constant of the pump's required NPSH curve & 1.17 (no units)\vspace{.6mm}\\
%$C_\text{p}$ & Specific heat at constant pressure & $1.013\mathrm{e}{-3}$ [$\frac{\text{MJ}}{\text{kg}\text{\celsius}}$] \vspace{.6mm} \\
%$c_\text{pump}$ & Unit conversion factor for pump flow rate & $6.31\mathrm{e}{-5}$ [$\frac{\frac{m^3}{gal}}{\frac{s}{min}}$] \vspace{.6mm} \\
%
$d$ & Elevation of rooftop vegetation relative to the cistern & 16 [m] \vspace{.6mm}\\
$D$ & Diameter of pipe & 0.2 [m] \vspace{.6mm}\\
$\Delta_\text{pump}$ & Magnitude of slope of pump performance equation & 5400 [$\frac{m}{\frac{m^3}{s}}$] \vspace{.6mm}\\
%
%$e_\text{s}$ & Mean saturation vapour pressure derived from air temperature & kPa \vspace{.6mm}\\
%$e_\text{a}$ & Actual vapour pressure derived from relative humidity & kPa \vspace{.6mm}\\
%$\epsilon$ & Ratio molecular weight of water vapour & 0.622 \vspace{.6mm}\\
%
$f$ & Friction factor of pipe system & $\approx$3.55 \vspace{.6mm}\\
%
$\tilde{g}$ & Acceleration due to gravity & 9.81 $\frac{\text{m}}{\text{s}^2}$ \vspace{.6mm}\\
%$G$ & Soil heat flux density & 0.4 $\frac{\text{MJ}}{\text{m}^2\text{day}}$\vspace{.6mm}\\
%
%$h$ & Humidity ratio of air & \text{From Toronto weather} \vspace{.6mm} \text{data \cite{canada_2021}} \vspace{.6mm}\\
%$h_\text{max}$ & Maximum humidity ratio of saturated air & 0.019826 at 25 \degree $C$ \vspace{.6mm}\\
$H_\text{pump,0}$ & Pump head in series at 0 flow rate & 59.7 m \vspace{.6mm}\\
%${k}_1$ & Water level in tank 1 & \vspace{.6mm}\\
%
%$\overline{k}_1$ & Maximum value of water level in tank 1 & 4 m \vspace{.6mm}\\
%
$k_\text{L}$ & Minor loss coefficient of system & 0.6 \vspace{.6mm}\\
%
$l$ & Length of pipe & 18.4 m \vspace{.6mm}\\
%$\lambda$ & Latent heat of vaporization & 2.45 
%$\frac{\text{MJ}}{\text{kg}}$ \vspace{.6mm}\\
%
$N$ & Length of discrete time horizon & 20 ($=$ 1 h) \vspace{.6mm}\\
%
%$P$ & Atmospheric pressure at 12 m above sea level & 101.16 kPa \vspace{.6mm}\\
$\tilde{\pi}$ & Circle circumference-to-diameter ratio & $\approx$3.14 \vspace{.6mm}\\
%
$r_\text{o}$ & Radius of outlet in cistern & $0.125$ m \vspace{.6mm}\\
%$R_\text{n}$ & Net radiation flux & \text{From Natural Resources} \vspace{.6mm} \text{Canada $\frac{\text{MJ}}{\text{m}^2\text{(day)}}$  \cite{canada_2020}} \vspace{.6mm}\\
%

$ \triangle \tau $ & Duration of $[t,t+1)$ & 3 min \vspace{.6mm}\\
%
%$v_\text{max}$ & Maximum operating speed of pump & 3450 rpm \vspace{.6mm}\\
%$v_\text{wind}$ & Wind speed & Stochastically generated $\frac{\text{m}}{\text{s}}$ \vspace{.6mm}\\
%$v_\text{air}$ & Velocity of air above water surface & 0.5 m/s \vspace{.6mm}\\
%
$z_\text{H}$ & Net positive suction head required in cistern & 2 m \\
$z_\text{o}$ & Elevation of outlet in cistern & 3 m \vspace{.6mm}\\
$z_\text{pump}$ & Pump elevation w.r.t base of cistern & 0.15 m \vspace{.6mm}\\
$z_\text{veg}$ & Minimum water balance required for rooftop vegetation & $4.57\mathrm{e}{-2}$ [m] \cite{melvin_yonts_2009} \vspace{.6mm} \\
%
\hline
\multicolumn{3}{p{251pt}}{m $=$ meter, s $=$ 
seconds, min $=$ minutes, h $=$ hours, rpm $=$ revolutions per minute, MJ $=$ mega-joules, kPa $=$ kilo-pascals.}
\end{tabular}
\label{tanksysinfo}
\end{table}

\begin{figure}[th]
% \the\columnwidth
\centerline{\includegraphics[width=\columnwidth]{cistern_rooftop3.png}}
\caption{Cistern Irrigation Model}
\label{exptfigure}
\end{figure}

\subsection{Smooth approximation of system equations}
A smooth transition is applied to equation (\ref{physics-out}) to permit continuity.
With all definitions following from section \ref{main-model}, we redefine the value of $X_{t+1}$ to be
\begin{equation}\label{linear}
x_{t+1} = x_t + f_{0}^{\epsilon}(x_t, u_t, w_t) \cdot \triangle\tau 
\end{equation}

Where $f_0^{\epsilon}(x_t,u_t,w_t)$ is smooth approximated $f_0(x_t,u_t,w_t)$.
\begin{equation}\label{physics}\begin{aligned}
f_0^{\epsilon}(x,u,w) & \coloneqq \left[ f_{01}^{\epsilon}(x,u,w), f_{02}^{\epsilon}(x,u,w) \right]^{T},\\
f_{01}^{\epsilon}(x,u,w) & \coloneqq  w - q_{\text{out}}^{\epsilon}(x_{1}) - q_\text{pump}^{\epsilon}(x,u),\\
f_{02}^{\epsilon}(x,u,w) & \coloneqq  w + q_\text{pump}^{\epsilon}(x,u)  - q_\text{evap}. 
\end{aligned}\end{equation}

First, from \eqref{physics-out}, we define a smooth approximation of $q_\text{out}(x_1)$ to be $q_\text{out}^{\epsilon}(x_1)$, where $\epsilon$ is a small positive real number.
\begin{subequations}\label{smooth}
\begin{equation}\label{smooth-physics-out}
%c_\text{out} & \coloneqq c_\text{d} \tilde{\pi} r_\text{o}^2 \sqrt{2 \tilde{g}}\\
q_\text{out}^{\epsilon}(x_1) := c_\text{out} \cdot \sqrt{\sigma_\text{out}^\epsilon(x_1)  \cdot x_1}
\end{equation}
where $\sigma_\text{out}^\epsilon(x_1)$ is smooth approximation of an indicator function for the condition $\frac{x_1}{a_1} \geq z_\text{o}$ \eqref{physics-out}. It is defined as the following:
\begin{subequations}
\begin{equation}
    \sigma_\text{out}^{\epsilon}(x_1) \coloneqq \frac{1}{1+\exp(\frac{x_1-\tilde{x}_\text{o1}}{\epsilon})}  \text{ ,}
\end{equation}
\begin{equation}
    \tilde{x}_\text{o1} = z_\text{o} \cdot a_1 \text{ ,}
\end{equation}
and $c_\text{out}$ is defined as:
\begin{equation}\label{cout}
c_\text{out} \coloneqq c_\text{d} \tilde{\pi} r_\text{o}^2 \sqrt{\frac{2\tilde{g}}{a_1}}
\end{equation}
\end{subequations}

Then, we define a smooth approximation of $q_\text{pump}$ as $q_\text{pump}^{\epsilon}$: \\
\begin{equation}
    q_\text{pump}^{\epsilon}(x,u) \coloneqq \frac{u}{v_\text{max}} \cdot \bar{q}_{\text{pump},v_{\text{max}}}^{\epsilon}(x) \;\;\text{,}
\end{equation}
where $\bar{q}_{\text{pump},v_{\text{max}}}^{\epsilon}(x)$ is the following:
\begin{equation}\label{q-epsilon}
%\bar{q}_{\text{pump},v_{\text{max}}}^{\epsilon}(x) \coloneqq \begin{cases} \sigma_\text{p1}(x_1) \cdot \frac{-\Delta_\text{pump} + \bar{q^{\epsilon}}(x_1)}{2c_1} & \text{if } \frac{x_2}{a_2}<z_\text{veg} \\ 0 & \text{otherwise} \end{cases},
\bar{q}_{\text{pump},v_{\text{max}}}^{\epsilon}(x) \coloneqq  \sigma_\text{p2}^\epsilon(x_2) \cdot \frac{-\Delta_\text{pump} + \bar{q^{\epsilon}}(x_1)}{2c_1} \;\; \text{,}
\end{equation}

$\sigma_\text{p2}^\epsilon(x_2)$ is a smooth approximation of an indicator function for the $\frac{x_2}{a_2} \geq z_\text{veg}$ condition, which is defined as:
\begin{subequations}
\begin{equation}
    \sigma_\text{p2}^\epsilon(x_2) \coloneqq \frac{1}{1+\exp{(\frac{x_2-\tilde{x}_\text{p2}}{\epsilon}})} \text{ ,}
\end{equation}
\begin{equation}
    \tilde{x}_\text{p2} = z_\text{veg}\cdot a_2 \text{ .}
\end{equation}
\end{subequations}
$\bar{q^{\epsilon}}(x_1)$ is defined as:
\begin{equation}
    \bar{q^{\epsilon}}(x_1) \coloneqq \sqrt{\Delta_{\text{pump}}^2-4c_1 \cdot \sigma_\text{p1}^\epsilon(x_1) \cdot (d-H_\text{pump,0}-\frac{x_1}{a_1})} \;\;,
\end{equation}
where $\sigma_\text{p1}^\epsilon(x_1)$ is a smooth approximation of an indicator function for the $\frac{x_1}{a_1}-z_\text{pump} < z_\text{H}$ condition \eqref{physics-pump}. It is defined as:
\begin{subequations}
\begin{equation}
    \sigma_\text{p1}^\epsilon(x_1) \coloneqq \frac{1}{1+\exp({\frac{\tilde{x}_\text{p1}-x_1}{\epsilon}})} \text{ ,}
\end{equation}
\begin{equation}
    \tilde{x}_\text{p1} = (z_\text{H}+z_\text{pump}) \cdot a_1 \text{ .}
\end{equation}
\end{subequations}

\end{subequations}

%We can write $\bar{q}_{\text{pump},v_{\text{max}}}^{\epsilon}(x)$ equivalently as follows. Let $I_{\{\frac{x_2}{a_2}<z_\text{veg}\}}(x_2) = 1$ if $\frac{x_2}{a_2}<z_\text{veg}$ and $I_{\{\frac{x_2}{a_2}<z_\text{veg}\}}(x_2) = 0$ otherwise. Then, we have
%\begin{equation}
%    \bar{q}_{\text{pump},v_{\text{max}}}^{\epsilon}(x) = I_{\{\frac{x_2}{a_2}<z_\text{veg}\}}(x_2) \cdot \sigma_\text{p}(x_1) \cdot \frac{-\Delta_\text{pump} + \bar{q^{\epsilon}}(x_1)}{2c_1}. 
%\end{equation}
% tilde_x
% tilde_u

\subsection{Linearization of smoothed system equations}
The goal of linearization is to write dynamics of the form
\begin{subequations}\label{linmodel}
\begin{equation}
    \tilde x_{t+1} = A_p \tilde x_t+ B_p \tilde u_t+ C_p\tilde w_t,
\end{equation}
where $p \coloneqq (\bar{x_1}, \bar{x_2}, \bar{u}, \bar{w})$ is a current operating point, and the variables $\tilde x$, $\tilde u$, and $\tilde w$ are defined in terms of $(\bar{x_1}, \bar{x_2}, \bar{u}, \bar{w})$ as follows: 
\begin{equation}
    \tilde x  \coloneqq x - \bar{x}, \;\;\;  \tilde u  \coloneqq u - \bar{u}, \;\;\; \tilde w  \coloneqq w - \bar{w}.
\end{equation}

Let $p \coloneqq (\bar{x_1}, \bar{x_2}, \bar{u}, \bar{w})$ be fixed. Also, let $u = \bar{u}$ and $w = \bar{w}$. Let $(A_p, B_p, C_p)$ be the linearization of the model about the point $(\bar{x_1}, \bar{x_2}, \bar{u}, \bar{w})$: 
\begin{equation}
\left.
A_\text{p} =
\begin{bmatrix}
    \frac{\partial f_{01}}{\partial x_1} &  \frac{\partial f_{01}}{\partial x_2} \\
    \frac{\partial f_{02}}{\partial x_1} &  \frac{\partial f_{02}}{\partial x_2}
\end{bmatrix}
\right|_{p}
\text{, } 
\left.
B_\text{p} = 
\begin{bmatrix}
    \frac{\partial f_{01}}{\partial u}\\
    \frac{\partial f_{02}}{\partial u}
\end{bmatrix}
\right|_{p}
\text{, }
\left.
C_\text{p} = 
\begin{bmatrix}
    \frac{\partial f_{01}}{\partial w}\\
    \frac{\partial f_{02}}{\partial w}
\end{bmatrix}
\right|_{p}
\end{equation}

\end{subequations}

Let $a$ be a fixed number (e.g., $a = 100$ m\textsuperscript{3}). We want to plot:
\begin{enumerate}
    \item $g_{\text{L}}(x) \coloneqq \bar{x} + A_p \tilde x+ B_p \tilde u+ C_p\tilde w$ versus $x \in [\bar{x}-a, \bar{x}+a]$,
    % \item $g_{\text{L}}(x) \coloneqq g_{\text{N}}(\bar{x}) + A_p \tilde x+ B_p \tilde u+ C_p\tilde w$ versus $x \in [\bar{x}-a, \bar{x}+a]$,
    \item $g_{\text{N}}(x) \coloneqq x + f_0^\epsilon(x, u, w) \Delta \tau$ versus $x \in [\bar{x}-a, \bar{x}+a]$.
    % \item $g_{\text{N}}(x) f_0^\epsilon(x, u, w) \Delta \tau$ versus $x \in [\bar{x}-a, \bar{x}+a]$.
\end{enumerate}
We repeat the above procedure for different choices of $\bar{x}$.

\begin{figure}[th]
% \the\columnwidth
\centerline{\includegraphics[width=\columnwidth]{pump_linear_vs_nonlinear/f01_50.jpg}}
\caption{Linearized model centered around p = (50, 0.04, 0.5, 20)}
\label{linearize-fig-1}
\end{figure}
\begin{figure}[th]
% \the\columnwidth
\centerline{\includegraphics[width=\columnwidth]{pump_linear_vs_nonlinear/f01_100.jpg}}
\caption{Linearized model centered around p = (100, 0.04, 0.5, 20)}
\label{linearize-fig-2}
\end{figure}
\begin{figure}[th]
% \the\columnwidth
\centerline{\includegraphics[width=\columnwidth]{pump_linear_vs_nonlinear/f01_200.jpg}}
\caption{Linearized model centered around p = (200, 0.04, 0.5, 20)}
\label{linearize-fig-3}
\end{figure}


\section{Model predictive control algorithm}
Let $t = 0$, $\bar{x}$ be the state at time $0$, $\bar{u}$ be the control at time $0$, and $\bar{w}$ be the disturbance at time $0$. Let $N \in \mathbb{N}$ and $M \in \mathbb{N}$ be given. For $t = 0, 1, \dots $, repeat the following steps:
\begin{enumerate}
    \item Linearize the model around $p \coloneqq (\bar{x},\bar{u},\bar{w})$ to obtain the matrices $A_p$, $B_p$, $C_p$ \eqref{linmodel}.
    \item  Find $(\tilde w_t, \tilde w_{t+1},...,\tilde w_{t+N})$ from the forecast.
    \item  Find $(\tilde u_j)_{j = t}^{t+N} := (\tilde u_t,\tilde u_{t+1},..., \tilde u_{t+N})$ to minimize the cost 
    \begin{subequations}
    \begin{equation}\label{cost}
        J((\tilde u_j)_{j = t}^{t+N}) := \sum_{i=t}^{t+N} ( \tilde x_{i2}/a_2 -  \tilde z_\text{veg})^2 + \lambda \tilde u_i^2,
    \end{equation}
    subject to 
    \begin{equation}\label{objective}
        \tilde x_{i+1} = A_p \tilde x_i + B_p \tilde u_i + C_p \tilde w_i \;\;\; i = t, t+1,...,t+N.
    \end{equation}
    \end{subequations}
    \item Apply $u_t = \tilde u_t + \bar{u}$.
     \item Proceed to the next time step, i.e., update $t$ by 1.
     \item Update $(\bar{x},\bar{u},\bar{w})$. Choose $\bar{x}$ to be the current state. $\bar{u} = u_t$. $\bar{w}$ is the average disturbance during several previous time points. If $t \geq M$, then $\bar{w} = \frac{1}{M+1}\sum_{j = t-M}^t w_j$. Otherwise, choose  $\bar{w} = \frac{1}{t}\sum_{j = 0}^{t-1} w_j$ to be the average over the previous time steps.
    \item Proceed to step 1 if $t < M$.
\end{enumerate}

\subsection{Rewrite problem of interest in standard form}
The problem of interest is outlined in step 3) (equations \ref{cost}-\ref{objective}). We want to rewrite the cost function (\ref{cost}) and objective function (\ref{objective}) in the standard form to solve for the optimal control input, $u_{t}$.

First, we define:
\begin{equation}\label{y_i}
    y_\text{i} \coloneqq \begin{bmatrix}y_\text{i1} \\ y_\text{i2}\end{bmatrix} \coloneqq \frac{1}{a_2} \begin{bmatrix}\tilde{x}_\text{i1}\\\tilde{x}_\text{i2}\end{bmatrix} - \begin{bmatrix}0 \\ \tilde{z}_\text{veg}\end{bmatrix} \coloneqq \frac{\tilde{x}_\text{i}}{a_2} - s \\\text{ where } \\
    s \coloneqq \begin{bmatrix}0 \\ \tilde{z}_\text{veg}\end{bmatrix} \text{, and}
\end{equation}
\begin{equation}\label{Q}
    Q \coloneqq \begin{bmatrix}0 & 0\\0 & 1\end{bmatrix} \text{, } Q_\text{f} = Q \text{.}
\end{equation}
Where we substitute (\ref{y_i}) into (\ref{objective}) to obtain:
\begin{subequations}
\begin{equation}\label{dynamics_bar}
    y_\text{i+1}=\bar{A}_\text{p}y_\text{i} + \bar{B}_\text{p}\tilde{u}_\text{i} + \bar{C}_\text{p}\tilde{w}_\text{i} + \bar{b}
\end{equation}
\begin{equation}
    \bar{A}_\text{p} \coloneqq A_\text{p} \text{, } \bar{B}_\text{p} \coloneqq \frac{B_\text{p}}{a_2} \text{, } \bar{C}_\text{p} \coloneqq \frac{C_\text{p}}{a_2} \text{, } \bar{b} \coloneqq (A_\text{p}-I_2)z_\text{veg} \text{, }
\end{equation}
where $I_2$ is a 2$\times$2 identity matrix.
\end{subequations}
\begin{subequations}
Then, we compose a compact matrix from the dynamics \ref{dynamics_bar} to form:
\begin{equation}\label{Y}
    Y = \tilde{A} y_\text{t} + \tilde{B} \tilde{U} + \tilde{C} \tilde{W} + \tilde{d}  \text{, }
\end{equation}
where $\tilde{A}$, $\tilde{B}$, $\tilde{C}$, $\tilde{d}$, $\tilde{U}$ and $\tilde{W}$ are defined:
\begin{equation}
\begin{gathered}
    \tilde{A} \coloneqq \begin{bmatrix}
        \bar{A}_{p} \\ (\bar{A})^2 \\ \vdots \\ (\bar{A}_{p})^N
    \end{bmatrix} \text{, } \\
    \tilde{B} \coloneqq \begin{bmatrix}
        \bar{B}_{p} & 0 & \dots & 0 \\
        \bar{A}_{p} \bar{B}_\text{p} & \bar{B}_{p} & \dots & 0 \\
        \vdots & \vdots & \ddots & \vdots \\
        \bar{A}_{p}^{N-1} \bar{B}_{p} & \bar{A}_{p}^{N-2} \bar{B}_{p} & \dots & \bar{B}_{p}
    \end{bmatrix} \text{, } \\
    \tilde{C} \coloneqq \begin{bmatrix}
        \bar{C}_{p} & 0 & \dots & 0 \\
        \bar{A}_{p} \bar{C}_{p} & \bar{C}_{p} & \dots & 0 \\
        \vdots & \vdots & \ddots & \vdots \\
        \bar{A}_{p}^{N-1} \bar{C}_{p} & \bar{A}_{p}^{N-2} \bar{C}_{p} & \dots & \bar{C}_{p}
    \end{bmatrix} \text{, }\\
    \tilde{d} \coloneqq \begin{bmatrix}
        I_2 & 0 & \dots & 0 \\
        \bar{A}_{p} & I_{2} \dots & 0\\
        \vdots & \vdots & \ddots & \vdots \\
        \bar{A}^{N-1}_{p} & \bar{A}^{N-2}_{p} & \dots & I_{2}
    \end{bmatrix}
    \begin{bmatrix}
        \bar{b} \\ \bar{b} \\ \vdots \\ \bar{b}
    \end{bmatrix}  \text{, }\\
    \tilde{U} \coloneqq \begin{bmatrix}
        \tilde{u}_{t} \\ \vdots \\ \tilde{u}_{t+N-1}
    \end{bmatrix} \text{, }
    \tilde{W} \coloneqq \begin{bmatrix}
        \tilde{w}_t \\ \tilde{w}_{t+1} \\ \vdots \\ \tilde{w}_{t+N-1}
    \end{bmatrix}
\end{gathered}
\end{equation}
\end{subequations}
\begin{subequations}

Then, we substitute (\ref{Y}) and (\ref{Q}) into (\ref{cost}), to obtain a compact matrix form of $J(\tilde{U})$:
\begin{equation}\label{cost_tilde}
    J(\tilde{U}) \coloneqq Y^\intercal \tilde{Q} Y + \tilde{U}^\intercal \tilde{R} \tilde{U} 
\end{equation} \text{,}
\text{where the matrices are defined as the following:}
\begin{equation}
\begin{gathered}
    Y \coloneqq \begin{bmatrix}
        y_\text{t+1} \\ y_\text{t+2} \\ \vdots \\ y_\text{t+N}
    \end{bmatrix} \text{, } 
    \tilde{Q} \coloneqq \begin{bmatrix}
        Q & & \\ & \ddots & \\ & & Q_\text{f}
    \end{bmatrix} \text{, and} \\
    \tilde{R} \coloneqq \begin{bmatrix}
        R & & \\ & \ddots & \\ & & R
    \end{bmatrix} \text{, } R \coloneqq \lambda
\end{gathered}
\end{equation}
\end{subequations}
Having (\ref{cost_tilde}) developed, we can now solve for the optimal control input by finding a $\tilde{U}$ that satisfies:
\begin{equation}
    \nabla J(\tilde{U}) = 0
\end{equation}



Some notes:
\begin{itemize}
    \item  The parameter $\lambda \geq 0$ is chosen to trade-off the desire to keep $\tilde x_{i2}/a_2$ close to $z_\text{veg}$ (so that the plants have enough water) and to conserve energy that is used by the pump ($|u_i|$ higher means that the pump requires more energy to operate).
    \item Compare the cost \eqref{cost} that we get from the algorithm above to a simple/baseline controller (if it will rain today with 80\% probability, then do not pump. Otherwise, pump water at a constant rate.)
\end{itemize}


==> revisions/my_file_v3.tex <==
The system consists of an underground cistern and a green roof. A pumping system is used to deliver water stored in the cistern to irrigate the green roof. Firstly, a mathematical model of the system was identified based on Newtonian physics. Then, the model was smoothly approximated to permit continuity. 

\subsection{Dynamic System Model}\label{dynamic-system-section}
In this paper, the dynamic system is the flow of water from the cistern to the green roof, where the water flow is controlled by a pump. The dynamic system model is a simplified abstraction of the real system (Fig. \ref{dynamic-system-fig}), where the two components - the cistern and the green roof are modelled as two tanks, tank 1 and tank 2 respectively. The model considers the mass balance of water entering and leaving tank 1 and tank 2. For tank 1, the source of water inflow is the storm water that enters through an inflow pipe $w_\text{r1}$. The water leaves tank 1 when the height of water exceeds $z_\text{o}$, where $q_\text{out}$ describes the volumetric flow rate of the water flowing out of tank 1 through the outlet. For tank 2, the sources of water inflow includes the surface runoff $w_\text{r2}$ and the irrigation $q_\text{pump}$. The outflow of tank 2 is modelled as the evapotranspiration rate $w_\text{e}$ and the water drained out of the vegetation due to soil capacity limits, $q_\text{drain}$. The model parameters and variables are defined in Table \ref{table-params}. 
Let $t \in \mathbb{T} := \{0,1,...,N-1\}$ be given. If $x_t \in S$, $u_t \in A$, $w_{r,t} \in \mathbb{R}$, and $w_{e,t} \in \mathbb{R}$ are the values of $X_t$, $U_t$, $W_{r,t}$, and $W_{e,t}$ respectively, then the value of $X_{t+1}$ is given by
\begin{equation}\begin{aligned}
    x_{t+1} = x_t + f_0(x_t,u_t,w_t)\cdot \triangle\tau,
\end{aligned}\end{equation}
such that if $x_{t+1,i} \geq \overline{k}_i$, then we redefine $x_{t+1,i} \coloneqq \overline{k}_i$, where $x_\text{t,i} \in [0, \overline{k}_{i}]$ (m\textsuperscript{3}) is the water volume of tank $i$. $u_{t} \in [0, \inf)$ is a pump setting, which is a value of $U_t$. $w_{r1,t} \in \mathbb{R}$ and $w_{r2,t} \in \mathbb{R}$ are values of the random disturbance $W_{r1,t}$ and $W_{r2,t}$ respectively. They represent the surface runoff that enters the system during the storm. $w_{e,t} \in \mathbb{R}$ is a value of another random disturbance $W_{e,t}$, representing the evapotranspiration rate of the plants on the green roof due to solar irradiance and other natural climate factors \cite{zotarelli2010step}.
The function $f_0 : \mathbb{R}_+^2 \times A \times \mathbb{R} \rightarrow \mathbb{R}_+^2$ is chosen according to simplified Newtonian physics:
\begin{equation}\label{system}\begin{aligned}
f_0(x,u,w_{r},w_{e}) & \coloneqq \left[ f_{01}(x,u,w_{r}), f_{02}(x,u,w_{r},w_{e}) \right]^\intercal,\\
f_{01}(x,u,w_{r}) & \coloneqq  w_{r1} - q_{\text{out}}(x_{1}) - q_\text{pump}(x,u),\\
f_{02}(x,u,w_{r},w_{e}) & \coloneqq  w_{r2} + q_\text{pump}(x,u)  - w_\text{e} - q_\text{drain}\\
\end{aligned}\end{equation}

We will define $q_\text{out}$, $q_\text{pump}$, $q_\text{drain}$, subsequently.

The cistern is equipped with an outlet that allows water to drain down via gravity when its water level reaches $z_\text{o}$, and an inlet that allows water to enter it. The flow rate of the water leaving the cistern via the outlet is defined by $q_\text{out}$, with an outlet radius $r_\text{o}$ and elevation $z_\text{o}$.
\begin{equation}\label{qout}
\begin{aligned}
q_\text{out}(x_{1}) &:= \begin{cases} c_\text{d} \tilde{\pi} r_\text{o}^2 \sqrt{2 \tilde{g} \frac{x_{1}}{a_{1}}}, & \text{if } \frac{x_{1}}{a_{1}} \geq z_o \\0 & \text{otherwise} \end{cases},\\
\end{aligned}
\end{equation}

Let $t \in \mathbb{T} := \{0,1,...,N-1\}$ be given. If $x_t \in S$, $u_t \in A$, $w_{r,t} \in \mathbb{R}$, and $w_{e,t} \in \mathbb{R}$ are the values of $X_t$, $U_t$, $W_{r,t}$, and $W_{e,t}$ respectively, then the value of $X_{t+1}$ is given by
\begin{subequations}\label{dynwater}
\begin{equation}\begin{aligned}
    x_{t+1} = x_t + f_0(x_t,u_t,w_t)\cdot \triangle\tau,
\end{aligned}\end{equation}
such that if $x_{t+1,i} \geq \overline{k}_i$, then we redefine $x_{t+1,i} \coloneqq \overline{k}_i$, where $x_\text{t,i} \in [0, \overline{k}_{i}]$ (m\textsuperscript{3}) is the water volume of tank $i$. $u_{t} \in [0, v_\text{max}]$ is a pump setting, which is a value of $U_t$. $w_{r,t} \in \mathbb{R}$ is a value of the random disturbance $W_{r,t}$, representing surface runoff that enters the system during the storm. $w_{e,t} \in \mathbb{R}$ is a value of another random disturbance $W_{e,t}$, representing the evapotranspiration rate of the plants on the green roof due to solar irradiance and other natural climate factors \cite{zotarelli2010step}.

The function $f_0 : \mathbb{R}_+^2 \times A \times \mathbb{R} \rightarrow \mathbb{R}_+^2$ is chosen according to simplified Newtonian physics:
\begin{equation}\label{physics-smooth}\begin{aligned}
f_0(x,u,w) & \coloneqq \left[ f_{01}(x,u,w), f_{02}(x,u,w) \right]^{T},\\
f_{01}(x,u,w) & \coloneqq  w_{r} - q_{\text{out}}(x_{1}) - q_\text{pump}(x,u),\\
f_{02}(x,u,w) & \coloneqq  w_{r} + q_\text{pump}(x,u)  - w_\text{e} - q_\text{drain}\\
\end{aligned}\end{equation}

We will define $q_\text{out}$, $q_\text{pump}$, $q_\text{drain}$, subsequently. Please refer to Table I for a list of model parameters.

The cistern is equipped with an outlet that allows water to drain down via gravity when its water level reaches $z_\text{o}$. The flow rate of the water leaving the cistern via the outlet is defined by $q_\text{out}$, with an outlet radius $r_\text{o}$ and elevation $z_\text{o}$.
\begin{equation}\label{physics-out}\begin{aligned}
q_\text{out}(x_{1}) &:= \begin{cases} c_\text{d} \tilde{\pi} r_\text{o}^2 \sqrt{2 \tilde{g} \frac{x_{1}}{a_{1}}}, & \text{if } \frac{x_{1}}{a_{1}} \geq z_o \\0 & \text{otherwise} \end{cases},\\
\end{aligned}\end{equation}

The flow rate of the pump, $q_\text{pump}(x,u)$, is derived from linear approximations of pump performance curves as well as the total head loss of the system. The system has pumps arranged in series to pump water from the cistern to the rooftop vegetation, therefore the slope of the linear approximated pump performance curves were doubled. The total head loss of the system is defined as the sum of the total static head loss, friction head loss, and the minor losses in the pipe system. The total static head loss is the total vertical distance that the water is raised by the pump. The friction head loss and minor head loss were determined based on the geometry and size of the pipe system, using the equation given in \cite[Eq. 6.79, p. 389]{white2011fluid}. 
The expression for $q_\text{pump}(x,u)$ is given by (\ref{physics-pump}), where $u$ is the control input that governs the speed of pump, $z_\text{H}$ is the required net positive suction head of the pump, and $z_\text{veg}$ is the minimum water balance required in the rooftop vegetation soil. 

\begin{subequations}\label{qpump}
\begin{equation}\label{physics-pump}\begin{aligned}
q_{\text{pump}}(x,u) &:= \begin{cases} 0 & \text{if }
\frac{x_{2}}{a_{2}} \geq z_\text{veg} \text{ or} \\ 
\text{} & \frac{x_{1}}{a_{1}} - z_\text{pump} < z_\text{H}\\
u \cdot \bar{q}_{\text{pump},0}(x) & \text{otherwise} \end{cases} \\
\end{aligned}\end{equation}

\begin{equation}\label{physics-pump-sub}\begin{aligned}
\bar{q}_{\text{pump},0}(x) & \coloneqq \frac{-\Delta_\text{pump}+ \sqrt{\Delta_\text{pump}^2-4c_{1}(d- \frac{x_{1}}{a_{1}}-H_\text{pump,0})}}{2c_{1}}\\
c_{1} & \coloneqq \frac{f \frac{l}{D} + k_\text{L}}{2 \tilde{g} a_{\text{pump}}} \\
\end{aligned}\end{equation}
\end{subequations}

For tank 2, water in the soil will be drained out when the soil reaches its capacity limit. This phenomenon is modelled with $q_\text{drain}$ using Darcy's Law \cite{selker_or_2018}: 
\begin{equation}\label{qdrain}\begin{aligned}
    q_\text{drain}(x_2) \coloneqq \begin{cases} 0 & \text{if }
    x_2 \cdot a_2 < z_\text{cap} \\
    K \cdot \frac{\frac{x_2}{a_2} + z_\text{soil}}{z_\text{soil}} & \text{ otherwise,} \end{cases}\\
\end{aligned}\end{equation}
where $K$ is the saturated hydraulic conductivity, and $z_\text{soil}$ the depth of the soil on the green roof.\\

\end{subequations}
%
Table \ref{tanksysinfo} lists model parameters.

\begin{table}[ht]
\caption{Stormwater System Parameters (Baseline)}
\label{table}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{|p{25pt}|p{125pt}|p{63pt}|}
\hline
\textbf{Symbol} &  \textbf{Description} & \textbf{Value} \vspace{.5mm}\\
\hline
$a_1$ & Bottom surface area of cistern & 70 m\textsuperscript{2} \vspace{.6mm}\\
$a_2$ & Bottom surface area of rooftop vegetation& 68.8 m\textsuperscript{2} \vspace{.6mm}\\
$a_\text{pump}$ & Area of flow through pump & 0.01 $\tilde{\pi}$ m\textsuperscript{2} \vspace{.6mm}\\
%
$c_\text{d}$ & Discharge coefficient & 0.61 (no units) \vspace{.6mm}\\
$c_\text{H,1}$ & Constant of the pump's required NPSH curve & 2.288 (no units)\vspace{.6mm}\\
$c_\text{H,2}$ & Constant of the pump's required NPSH curve & 1.17 (no units)\vspace{.6mm}\\
$d$ & Elevation of rooftop vegetation relative to the cistern & 16 m \vspace{.6mm}\\
$D$ & Diameter of pipe & 0.2 m \vspace{.6mm}\\
$\Delta_\text{pump}$ & Magnitude of slope of pump performance equation & 5400 $\frac{m}{\frac{m^3}{s}}$ \vspace{.6mm}\\
$f$ & Friction factor of pipe system & $\approx$3.55 \vspace{.6mm}\\
%
$\tilde{g}$ & Acceleration due to gravity & 9.81 $\frac{\text{m}}{\text{s}^2}$ \vspace{.6mm}\\
$H_\text{pump,0}$ & Pump head in series at 0 flow rate & 59.7 m \vspace{.6mm}\\
$K$ & Saturated hydraulic conductivity & 7.83e-8 m/s \cite{al-kharabsheh_azzam_2019} \vspace{.6mm}\\
$k_\text{L}$ & Minor loss coefficient of system & 0.6 \vspace{.6mm}\\
%
$l$ & Length of pipe & 18.4 m \vspace{.6mm}\\
$N$ & Length of discrete time horizon & 20 ($=$ 1 h) \vspace{.6mm}\\
%
$\tilde{\pi}$ & Circle circumference-to-diameter ratio & $\approx$3.14 \vspace{.6mm}\\
%
$r_\text{o}$ & Radius of outlet in cistern & $0.125$ m \vspace{.6mm}\\
$ \triangle \tau $ & Duration of $[t,t+1)$ & 1 min \vspace{.6mm}\\
$z_\text{cap}$ & Soil capacity &  $0.05 \cdot a_2$ $\text{m}^3$ \vspace{.6mm}\\
$z_\text{H}$ & Net positive suction head required for the pump & 1 m \\
$z_\text{o}$ & Elevation of outlet in cistern & 3 m \vspace{.6mm}\\
$z_\text{pump}$ & Pump elevation w.r.t base of cistern & 0.15 m \vspace{.6mm}\\
$z_\text{soil}$ & Soil depth on green roof & 0.5 m \vspace{.6mm} \\
$z_\text{veg}$ & Minimum water balance required for rooftop vegetation & $4.57\mathrm{e}{-2}$ m \cite{melvin_yonts_2009} \vspace{.6mm} \\
%
\hline
\multicolumn{3}{p{251pt}}{m $=$ meter, s $=$ 
seconds, min $=$ minutes, h $=$ hours, rpm $=$ revolutions per minute, MJ $=$ mega-joules, kPa $=$ kilo-pascals.}
\end{tabular}
\label{tanksysinfo}
\end{table}

\begin{figure}[th]
% \the\columnwidth
\centerline{\includegraphics[width=\columnwidth]{cistern_rooftop3.png}}
\caption{Cistern Irrigation Model}
\label{exptfigure}
\end{figure}

\subsection{Smooth approximation of system equations}
A smooth transition is applied to equation (\ref{physics-out}) and (\ref{physics-pump}) to permit continuity.
With all definitions following from section \ref{main-model}, we redefine the value of $X_{t+1}$ to be
\begin{equation}\label{linear}
x_{t+1} = x_t + f_{0}^{\epsilon}(x_t, u_t, w_t) \cdot \triangle\tau 
\end{equation}

Where $f_0^{\epsilon}(x_t,u_t,w_t)$ is smooth approximated $f_0(x_t,u_t,w_t)$.
\begin{equation}\label{physics}\begin{aligned}
f_0^{\epsilon}(x,u,w) & \coloneqq \left[ f_{01}^{\epsilon}(x,u,w), f_{02}^{\epsilon}(x,u,w) \right]^{T},\\
f_{01}^{\epsilon}(x,u,w) & \coloneqq  w_r - q_{\text{out}}^{\epsilon}(x_{1}) - q_\text{pump}^{\epsilon}(x,u),\\
f_{02}^{\epsilon}(x,u,w) & \coloneqq  w_r + q_\text{pump}^{\epsilon}(x,u)  - w_\text{e} - q_\text{drain}. 
\end{aligned}\end{equation}

First, from \eqref{physics-out}, we define a smooth approximation of $q_\text{out}(x_1)$ to be $q_\text{out}^{\epsilon}(x_1)$, where $\epsilon$ is a small positive real number.
\begin{subequations}\label{smooth}
\begin{equation}\label{smooth-physics-out}
q_\text{out}^{\epsilon}(x_1) := c_\text{out} \cdot \sqrt{\sigma_\text{out}^\epsilon(x_1)  \cdot x_1}
\end{equation}
where $\sigma_\text{out}^\epsilon(x_1)$ is smooth approximation of an indicator function for the condition $\frac{x_1}{a_1} \geq z_\text{o}$ \eqref{physics-out}. It is defined as the following:
\begin{subequations}
\begin{equation}
    \sigma_\text{out}^{\epsilon}(x_1) \coloneqq \frac{1}{1+\exp(\frac{x_1-\tilde{x}_\text{o1}}{\epsilon})}  \text{ ,}
\end{equation}
\begin{equation}
    \tilde{x}_\text{o1} = z_\text{o} \cdot a_1 \text{ ,}
\end{equation}
and $c_\text{out}$ is defined as:
\begin{equation}\label{cout}
c_\text{out} \coloneqq c_\text{d} \tilde{\pi} r_\text{o}^2 \sqrt{\frac{2\tilde{g}}{a_1}}
\end{equation}
\end{subequations}

Then, we define a smooth approximation of $q_\text{pump}$ as $q_\text{pump}^{\epsilon}$: \\
\begin{equation}
    q_\text{pump}^{\epsilon}(x,u) \coloneqq \frac{u}{v_\text{max}} \cdot \bar{q}_{\text{pump},v_{\text{max}}}^{\epsilon}(x) \;\;\text{,}
\end{equation}
where $\bar{q}_{\text{pump},v_{\text{max}}}^{\epsilon}(x)$ is the following:
\begin{equation}\label{q-epsilon}
\bar{q}_{\text{pump},v_{\text{max}}}^{\epsilon}(x) \coloneqq  \sigma_\text{p2}^\epsilon(x_2) \cdot \frac{-\Delta_\text{pump} + \bar{q^{\epsilon}}(x_1)}{2c_1} \;\; \text{,}
\end{equation}

$\sigma_\text{p2}^\epsilon(x_2)$ is a smooth approximation of an indicator function for the $\frac{x_2}{a_2} \geq z_\text{veg}$ condition, which is defined as:
\begin{subequations}
\begin{equation}
    \sigma_\text{p2}^\epsilon(x_2) \coloneqq \frac{1}{1+\exp{(\frac{x_2-\tilde{x}_\text{p2}}{\epsilon}})} \text{ ,}
\end{equation}
\begin{equation}
    \tilde{x}_\text{p2} = z_\text{veg}\cdot a_2 \text{ .}
\end{equation}
\end{subequations}
$\bar{q^{\epsilon}}(x_1)$ is defined as:
\begin{equation}
    \bar{q^{\epsilon}}(x_1) \coloneqq \sqrt{\Delta_{\text{pump}}^2-4c_1 \cdot \sigma_\text{p1}^\epsilon(x_1) \cdot (d-H_\text{pump,0}-\frac{x_1}{a_1})} \;\;,
\end{equation}
where $\sigma_\text{p1}^\epsilon(x_1)$ is a smooth approximation of an indicator function for the $\frac{x_1}{a_1}-z_\text{pump} < z_\text{H}$ condition \eqref{physics-pump}. It is defined as:
\begin{subequations}
\begin{equation}
    \sigma_\text{p1}^\epsilon(x_1) \coloneqq \frac{1}{1+\exp({\frac{\tilde{x}_\text{p1}-x_1}{\epsilon}})} \text{ ,}
\end{equation}
\begin{equation}
    \tilde{x}_\text{p1} = (z_\text{H}+z_\text{pump}) \cdot a_1 \text{ .}
\end{equation}
\end{subequations}

Similarly, $q_\text{drain}$ is smoothly approximated by $q_\text{drain}^{\epsilon}$:
\begin{equation}
    q_\text{drain}^{\epsilon}(x_2) \coloneqq K \frac{\frac{x_2(\frac{1}{1+\exp{\frac{(x_2-z_\text{soil} \cdot a_2)}{\epsilon}}})}{a_2} + z_\text{soil}}{z_\text{soil}}
\end{equation}
\end{subequations}

\subsection{Linearization of smoothed system equations}
The goal of linearization is to write dynamics of the form
\begin{subequations}\label{linmodel}
\begin{equation}
    \tilde x_{t+1} = A_p \tilde x_t+ B_p \tilde u_t+ C_p\tilde w_{r,t} + D_p \tilde w_{e,t},
\end{equation}
where $p \coloneqq (\bar{x_1}, \bar{x_2}, \bar{u}, \bar{w})$ is a current operating point, and the variables $\tilde x$, $\tilde u$, and $\tilde w$ are defined in terms of $(\bar{x_1}, \bar{x_2}, \bar{u}, \bar{w})$ as follows: 
\begin{equation}
    \tilde x  \coloneqq x - \bar{x}, \;\;\;  \tilde u  \coloneqq u - \bar{u}, \;\;\; \tilde w  \coloneqq w - \bar{w}.
\end{equation}

Let $p \coloneqq (\bar{x_1}, \bar{x_2}, \bar{u}, \bar{w_r}, \bar{w_e})$ be fixed. Also, let $u = \bar{u}$ and $w = \bar{w}$. Let $(A_p, B_p, C_p)$ be the linearization of the model about the point $(\bar{x_1}, \bar{x_2}, \bar{u}, \bar{w})$: 
\begin{equation}
\begin{gathered}
\left.
A_\text{p} =
\begin{bmatrix}
    \frac{\partial f_{01}}{\partial x_1} &  \frac{\partial f_{01}}{\partial x_2} \\
    \frac{\partial f_{02}}{\partial x_1} &  \frac{\partial f_{02}}{\partial x_2}
\end{bmatrix}
\right|_{p}
\text{, } 
\left.
B_\text{p} = 
\begin{bmatrix}
    \frac{\partial f_{01}}{\partial u}\\
    \frac{\partial f_{02}}{\partial u}
\end{bmatrix}
\right|_{p}
\text{, }
\left.
C_\text{p} = 
\begin{bmatrix}
    \frac{\partial f_{01}}{\partial w_r}\\
    \frac{\partial f_{02}}{\partial w_r}
\end{bmatrix}
\right|_{p} \\
\left.
D_\text{p} = 
\begin{bmatrix}
    \frac{\partial f_{01}}{\partial w_e}\\
    \frac{\partial f_{02}}{\partial w_e}
\end{bmatrix}
\right|_{p}
\end{gathered}
\end{equation}

\end{subequations}

Let $a$ be a fixed number (e.g., $a = 100$ m\textsuperscript{3}). We want to plot:
\begin{enumerate}
    \item $g_{\text{L}}(x) \coloneqq \bar{x} + A_p \tilde x+ B_p \tilde u+ C_p\tilde w_r + D_p \tilde w_e$ versus $x \in [\bar{x}-a, \bar{x}+a]$,
    % \item $g_{\text{L}}(x) \coloneqq g_{\text{N}}(\bar{x}) + A_p \tilde x+ B_p \tilde u+ C_p\tilde w$ versus $x \in [\bar{x}-a, \bar{x}+a]$,
    \item $g_{\text{N}}(x) \coloneqq x + f_0^\epsilon(x, u, w) \Delta \tau$ versus $x \in [\bar{x}-a, \bar{x}+a]$.
    % \item $g_{\text{N}}(x) f_0^\epsilon(x, u, w) \Delta \tau$ versus $x \in [\bar{x}-a, \bar{x}+a]$.
\end{enumerate}
We repeat the above procedure for different choices of $\bar{x}$.

\begin{figure}[th]
% \the\columnwidth
\centerline{\includegraphics[width=\columnwidth]{pump_linear_vs_nonlinear/f01_50.jpg}}
\caption{Linearized $f_{01}$ centered around p = (50, 0.04, 0.5, 20, 0.004)}
\label{linearize-fig-1}
\end{figure}
\begin{figure}[th]
% \the\columnwidth
\centerline{\includegraphics[width=\columnwidth]{pump_linear_vs_nonlinear/f01_100.jpg}}
\caption{Linearized $f_{01}$ centered around p = (100, 0.04, 0.5, 20, 0.004)}
\label{linearize-fig-2}
\end{figure}
\begin{figure}[th]
% \the\columnwidth
\centerline{\includegraphics[width=\columnwidth]{pump_linear_vs_nonlinear/f01_200.jpg}}
\caption{Linearized $f_{01}$ centered around p = (200, 0.04, 0.5, 20, 0.004)}
\label{linearize-fig-3}
\end{figure}


\section{Model predictive control algorithm}
Let $t = 0$, $\bar{x}$ be the state at time $0$, $\bar{u}$ be the control at time $0$, and $\bar{w}$ be the disturbance at time $0$. Let $N \in \mathbb{N}$ and $M \in \mathbb{N}$ be given. For $t = 0, 1, \dots $, repeat the following steps:
\begin{enumerate}
    \item Linearize the model around $p$ to obtain the matrices $A_p$, $B_p$, $C_p$, $D_p$ \eqref{linmodel}.
    \item  Find $(\tilde w_t, \tilde w_{t+1},...,\tilde w_{t+N})$ from the forecast.
    \item  Find $(\tilde u_j)_{j = t}^{t+N} := (\tilde u_t,\tilde u_{t+1},..., \tilde u_{t+N})$ to minimize the cost 
    \begin{subequations}
    \begin{equation}\label{cost}
        J((\tilde u_j)_{j = t}^{t+N}) := \sum_{i=t}^{t+N} ( \tilde x_{i2}/a_2 -  \tilde z_\text{veg})^2 + \lambda \tilde u_i^2,
    \end{equation}
    subject to 
    \begin{equation}\label{objective}
        \tilde x_{i+1} = A_p \tilde x_i + B_p \tilde u_i + C_p \tilde w_i \;\;\; i = t, t+1,...,t+N.
    \end{equation}
    \end{subequations}
    \item Apply $u_t = \tilde u_t + \bar{u}$.
     \item Proceed to the next time step, i.e., update $t$ by 1.
     \item Update $(\bar{x},\bar{u},\bar{w})$. Choose $\bar{x}$ to be the current state. $\bar{u} = u_t$. $\bar{w}$ is the average disturbance during several previous time points. If $t \geq M$, then $\bar{w} = \frac{1}{M+1}\sum_{j = t-M}^t w_j$. Otherwise, choose  $\bar{w} = \frac{1}{t}\sum_{j = 0}^{t-1} w_j$ to be the average over the previous time steps.
    \item Proceed to step 1 if $t < M$.
\end{enumerate}

\subsection{Rewrite problem of interest in standard form}
The problem of interest is outlined in step 3) (equations \ref{cost}-\ref{objective}). We want to rewrite the cost function (\ref{cost}) and objective function (\ref{objective}) in the standard form to solve for the optimal control input, $u_{t}$.

First, we define:
\begin{equation}\label{y_i}
    y_\text{i} \coloneqq \begin{bmatrix}y_\text{i1} \\ y_\text{i2}\end{bmatrix} \coloneqq \frac{1}{a_2} \begin{bmatrix}\tilde{x}_\text{i1}\\\tilde{x}_\text{i2}\end{bmatrix} - \begin{bmatrix}0 \\ \tilde{z}_\text{veg}\end{bmatrix} \coloneqq \frac{\tilde{x}_\text{i}}{a_2} - s \\\text{ where } \\
    s \coloneqq \begin{bmatrix}0 \\ \tilde{z}_\text{veg}\end{bmatrix} \text{, and}
\end{equation}
\begin{equation}\label{Q}
    Q \coloneqq \begin{bmatrix}0 & 0\\0 & 1\end{bmatrix} \text{, } Q_\text{f} = Q \text{.}
\end{equation}
Where we substitute (\ref{y_i}) into (\ref{objective}) to obtain:
\begin{subequations}
\begin{equation}\label{dynamics_bar}
    y_\text{i+1}=\bar{A}_\text{p}y_\text{i} + \bar{B}_\text{p}\tilde{u}_\text{i} + \bar{C}_\text{p}\tilde{w}_\text{r,i} + \bar{D}_\text{p}\tilde{w}_\text{e,i} + \bar{b} \text{,}
\end{equation}
where 
\begin{equation}
\begin{gathered}
    \bar{A}_\text{p} \coloneqq A_\text{p} \text{, } \bar{B}_\text{p} \coloneqq \frac{B_\text{p}}{a_2} \text{, } \bar{C}_\text{p} \coloneqq \frac{C_\text{p}}{a_2} \text{, } \bar{D}_\text{p} \coloneqq \frac{D_\text{p}}{a_2} \text{,}\\
    \bar{b} \coloneqq (A_\text{p}-I_2)z_\text{veg} \text{, }    
\end{gathered}
\end{equation}
and $I_2$ is a 2$\times$2 identity matrix.
\end{subequations}
\begin{subequations}
Then, we write the dynamics (\ref{dynamics_bar}) in the matrix form:
\begin{equation}\label{Y}
    Y = \tilde{A} y_\text{t} + \tilde{B} \tilde{U} + \tilde{C} \tilde{W_r} + \tilde{D} \tilde{W_e} + \tilde{d}  \text{, }
\end{equation}
where $\tilde{A}$, $\tilde{B}$, $\tilde{C}$, $\tilde{D}$, $\tilde{d}$, $\tilde{U}$,  $\tilde{W_r}$, and $\tilde{W_e}$ are defined:
\begin{equation}
\begin{gathered}
    \tilde{A} \coloneqq \begin{bmatrix}
        \bar{A}_{p} \\ (\bar{A})^2 \\ \vdots \\ (\bar{A}_{p})^N
    \end{bmatrix} \text{, } \\
    \tilde{B} \coloneqq \begin{bmatrix}
        \bar{B}_{p} & 0 & \dots & 0 \\
        \bar{A}_{p} \bar{B}_\text{p} & \bar{B}_{p} & \dots & 0 \\
        \vdots & \vdots & \ddots & \vdots \\
        \bar{A}_{p}^{N-1} \bar{B}_{p} & \bar{A}_{p}^{N-2} \bar{B}_{p} & \dots & \bar{B}_{p}
    \end{bmatrix} \text{, } \\
    \tilde{C} \coloneqq \begin{bmatrix}
        \bar{C}_{p} & 0 & \dots & 0 \\
        \bar{A}_{p} \bar{C}_{p} & \bar{C}_{p} & \dots & 0 \\
        \vdots & \vdots & \ddots & \vdots \\
        \bar{A}_{p}^{N-1} \bar{C}_{p} & \bar{A}_{p}^{N-2} \bar{C}_{p} & \dots & \bar{C}_{p}
    \end{bmatrix} \text{, }\\
    \tilde{D} \coloneqq \begin{bmatrix}
        \bar{D}_{p} & 0 & \dots & 0 \\
        \bar{A}_{p} \bar{D}_{p} & \bar{D}_{p} & \dots & 0 \\
        \vdots & \vdots & \ddots & \vdots \\
        \bar{A}_{p}^{N-1} \bar{D}_{p} & \bar{A}_{p}^{N-2} \bar{D}_{p} & \dots & \bar{D}_{p}
    \end{bmatrix} \text{, } \\
    \tilde{d} \coloneqq \begin{bmatrix}
        I_2 & 0 & \dots & 0 \\
        \bar{A}_{p} & I_{2} \dots & 0\\
        \vdots & \vdots & \ddots & \vdots \\
        \bar{A}^{N-1}_{p} & \bar{A}^{N-2}_{p} & \dots & I_{2}
    \end{bmatrix}
    \begin{bmatrix}
        \bar{b} \\ \bar{b} \\ \vdots \\ \bar{b}
    \end{bmatrix}  \text{, }\\
    \tilde{U} \coloneqq \begin{bmatrix}
        \tilde{u}_{t} \\ \vdots \\ \tilde{u}_{t+N-1}
    \end{bmatrix} \text{, }
    \tilde{W_r} \coloneqq \begin{bmatrix}
        \tilde{w}_{r,t} \\ \tilde{w}_{r,t+1} \\ \vdots \\ \tilde{w}_{r,t+N-1}
    \end{bmatrix} \text{,}\\
    \tilde{W_e} \coloneqq \begin{bmatrix}
        \tilde{w}_{e,t} \\ \tilde{w}_{e,t+1} \\ \vdots \\ \tilde{w}_{e,t+N-1}
    \end{bmatrix}
\end{gathered}
\end{equation}
\end{subequations}
\begin{subequations}

Then, we substitute (\ref{Y}) and (\ref{Q}) into (\ref{cost}), to obtain a compact matrix form of $J(\tilde{U})$:
\begin{equation}\label{cost_tilde}
    J(\tilde{U}) \coloneqq Y^\intercal \tilde{Q} Y + \tilde{U}^\intercal \tilde{R} \tilde{U} 
\end{equation} \text{,}
\text{where the matrices are defined as the following:}
\begin{equation}
\begin{gathered}
    Y \coloneqq \begin{bmatrix}
        y_\text{t+1} \\ y_\text{t+2} \\ \vdots \\ y_\text{t+N}
    \end{bmatrix} \text{, } 
    \tilde{Q} \coloneqq \begin{bmatrix}
        Q & & \\ & \ddots & \\ & & Q_\text{f}
    \end{bmatrix} \text{, and} \\
    \tilde{R} \coloneqq \begin{bmatrix}
        R & & \\ & \ddots & \\ & & R
    \end{bmatrix} \text{, } R \coloneqq \lambda
\end{gathered}
\end{equation}
\end{subequations}
Having (\ref{cost_tilde}) developed, we can now solve for the optimal control input by finding a $\tilde{U}$ that satisfies:
\begin{equation}
    \nabla J(\tilde{U}) = 0
\end{equation}

\section{}

Some notes:
\begin{itemize}
    \item  The parameter $\lambda \geq 0$ is chosen to trade-off the desire to keep $\tilde x_{i2}/a_2$ close to $z_\text{veg}$ (so that the plants have enough water) and to conserve energy that is used by the pump ($|u_i|$ higher means that the pump requires more energy to operate).
    \item Compare the cost \eqref{cost} that we get from the algorithm above to a simple/baseline controller (if it will rain today with 80\% probability, then do not pump. Otherwise, pump water at a constant rate.)
\end{itemize}

